A new formulation of compartmental epidemic modelling for arbitrary distributions of incubation and removal times

The paradigm for compartment models in epidemiology assumes exponentially distributed incubation and removal times, which is not realistic in actual populations. Commonly used variations with multiple exponentially distributed variables are more flexible, yet do not allow for arbitrary distributions. We present a new formulation, focussing on the SEIR concept that allows to include general distributions of incubation and removal times. We compare the solution to two types of agent-based model simulations, a spatially homogeneous one where infection occurs by proximity, and a model on a scale-free network with varying clustering properties, where the infection between any two agents occurs via their link if it exists. We find good agreement in both cases. Furthermore a family of asymptotic solutions of the equations is found in terms of a logistic curve, which after a non-universal time shift, fits extremely well all the microdynamical simulations. The formulation allows for a simple numerical approach; software in Julia and Python is provided.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CUSTOM COMMANDS

% Abbreviations for environment tags
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}

% References
\newcommand{\req}[1]{Eq.~(\ref{#1})}
\newcommand{\res}[1]{Section~\ref{#1}}
\newcommand{\reapp}[1]{Appendix~\ref{#1}}
\newcommand{\rep}[1]{\cite{#1}}
\newcommand{\refig}[1]{Fig.~\ref{#1}}
\newcommand{\ret}[1]{Table~\ref{#1}}

% Miscellaneous symbols
\newcommand{\dif}{{\rm d}}
\newcommand{\Tr}{{\rm Tr}}
\newcommand{\tr}{{\rm tr}}
\newcommand{\Pf}{{\rm Pf}}
\newcommand{\Id}{\mathbf{1}}
\newcommand{\pexp}{\mbox{P} \, \mbox{exp}}
\newcommand{\Per}[1]{\mathbf{S}_{#1}}
\newcommand{\eps}{\varepsilon}
\newcommand{\ci}[1]{\boldsymbol{#1}}
\renewcommand{\Re}[1]{{\mathcal Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{{\mathcal Im}\left\{#1\right\}}
\newcommand{\Dslash}{\relax{\kern+.25em / \kern-.70em D}}
\newcommand{\GF}{G_{\rm\scriptscriptstyle F}}
\newcommand{\alphas}{\alpha_{\rm\scriptscriptstyle s}}

\newcommand{\dl}{\stackrel{\leftarrow}{D}}
\newcommand{\dr}{\stackrel{\rightarrow}{D}}
\newcommand{\dcl}{\stackrel{\leftarrow}{\cD}}
\newcommand{\dcr}{\stackrel{\rightarrow}{\cD}}
\newcommand{\pdl}{\stackrel{\leftarrow}{\partial}}
\newcommand{\pdr}{\stackrel{\rightarrow}{\partial}}

\newcommand{\Dwd}{D_{\rm\scriptstyle w}}
\newcommand{\Dtwd}{D_{\rm\scriptstyle tw}}
\newcommand{\arcsinh}{\rm arcsinh}
\newcommand{\arccosh}{\rm arccosh}
\newcommand{\arctanh}{\rm arctanh}
\newcommand{\fm}{{\rm fm}}
\newcommand{\MeV}{{\rm MeV}}
\newcommand{\GeV}{{\rm GeV}}

% Numerical sets / Groups
\newcommand{\Real}{\relax{\mathsf{\Gamma\kern-.35em R}}}
\newcommand{\Int}{\relax{\mathsf{Z\kern-.40em Z}}}
\newcommand{\Ztwo}{Z_2}
\newcommand{\Zf}{Z_4}
\newcommand{\ZN}{Z_{\NC}}
\newcommand{\ZTN}{Z_{2\NC}}
\newcommand{\UO}{\mbox{U}(1)}
\newcommand{\SUT}{\mbox{SU}(2)}
\newcommand{\UT}{\mbox{U}(2)}
\newcommand{\SUt}{\mbox{SU}(3)}
\newcommand{\Ut}{\mbox{U}(3)}
\newcommand{\SUN}{\mbox{SU}(\NC)}
\newcommand{\UN}{\mbox{U}(\NC)}
\newcommand{\SUQ}{\mbox{SU}(Q)}
\newcommand{\UQ}{\mbox{U}(Q)}
\newcommand{\SU}{\mbox{SU}}
\newcommand{\CF}{C_{\rm F}}

% Scriptstyle fractions
\newcommand{\half}{{\scriptstyle{{1\over 2}}}}
\newcommand{\third}{{\scriptstyle{{1\over 3}}}}
\newcommand{\quart}{{\scriptstyle{{1\over 4}}}}
\newcommand{\sixth}{{\scriptstyle{{1\over 6}}}}
\newcommand{\eighth}{{\scriptstyle{{1\over 8}}}}
\newcommand{\sixteenth}{{\scriptstyle{{1\over 16}}}}
\newcommand{\twth}{{\scriptstyle{{1\over 12}}}}
\newcommand{\thalf}{{\scriptstyle{{3\over 2}}}}
\newcommand{\fhalf}{{\scriptstyle{{5\over 2}}}}
\newcommand{\tthird}{{\scriptstyle{{2\over 3}}}}
\newcommand{\fthird}{{\scriptstyle{{5\over 3}}}}
\newcommand{\ihalf}{{\scriptstyle{{i\over 2}}}}
\newcommand{\iquart}{{\scriptstyle{{i\over 4}}}}
\newcommand{\pihalf}{{\scriptstyle{{\pi\over 2}}}}
\newcommand{\oneovN}{{\scriptstyle{{1\over \NC}}}}

% Colours, flavours, susies
%\newcommand{\NC}{N_c}
\newcommand{\NC}{N}
\newcommand{\NF}{N_\mathrm{\scriptstyle f}}
\newcommand{\NSS}{{\cal N}}

% Renormalisation schemes
\newcommand{\MS}{{\rm MS}}
\newcommand{\MSbar}{{\overline{\rm MS}}}
\newcommand{\SF}{{\rm SF}}

% Renormalised, RGI and related quantities
\newcommand{\gbar}{\kern1pt\overline{\kern-1pt g\kern-0pt}\kern1pt}
\newcommand{\mbar}{\kern2pt\overline{\kern-1pt m\kern-1pt}\kern1pt}
\newcommand{\obar}[1]{\kern3pt\overline{\kern-2pt #1\kern-0pt}\kern1pt}
\newcommand{\gren}{g_{\rm R}}
\newcommand{\mren}[1]{m_{{\rm R} #1}}
\newcommand{\muren}[1]{\mu_{{\rm R} #1}}
\newcommand{\oren}[1]{#1_{\rm R}}
\newcommand{\lQCD}{\Lambda_{\rm\scriptscriptstyle QCD}}
\newcommand{\mrgi}{M}
\newcommand{\orgi}[1]{\hat #1}
\newcommand{\msubt}{m_{\rm q}}
\newcommand{\mcrit}{m_{\rm cr}}
\newcommand{\hopc}{\kappa_{\rm c}}
\newcommand{\muq}{\mu_{\rm q}}

% Correlation functions
\newcommand{\fX}{f_{\rm\scriptscriptstyle X}}
\newcommand{\fP}{f_{\rm\scriptscriptstyle P}}
\newcommand{\fS}{f_{\rm\scriptscriptstyle S}}
\newcommand{\fA}{f_{\rm\scriptscriptstyle A}}
\newcommand{\fV}{f_{\rm\scriptscriptstyle V}}
\newcommand{\kX}{k_{\rm\scriptscriptstyle X}}
\newcommand{\kA}{k_{\rm\scriptscriptstyle A}}
\newcommand{\kV}{k_{\rm\scriptscriptstyle V}}
\newcommand{\kT}{k_{\rm\scriptscriptstyle T}}
\newcommand{\hT}{h_{\rm\scriptscriptstyle T}}

% Z's, SSF's et rel.
\newcommand{\Zm}{Z_{\rm m}}
\newcommand{\ZP}{Z_{\rm\scriptscriptstyle P}}
\newcommand{\ZS}{Z_{\rm\scriptscriptstyle S}}
\newcommand{\ZA}{Z_{\rm\scriptscriptstyle A}}
\newcommand{\ZV}{Z_{\rm\scriptscriptstyle V}}
\newcommand{\ZT}{Z_{\rm\scriptscriptstyle T}}
\newcommand{\sigmaP}{\sigma_{\rm\scriptscriptstyle P}}
\newcommand{\sigmaT}{\sigma_{\rm\scriptscriptstyle T}}
\newcommand{\SigmaP}{\Sigma_{\rm\scriptscriptstyle P}}
\newcommand{\SigmaT}{\Sigma_{\rm\scriptscriptstyle T}}
\newcommand{\lmax}{L_{\rm max}}
\newcommand{\lmin}{L_{\rm min}}

% O(a) improvement
\newcommand{\Oa}{\mbox{O}(a)}
\newcommand{\Oasq}{\mbox{O}(a^2)}
\newcommand{\Ogsqa}{\mbox{O}(g_0^2 a)}
\newcommand{\Ogqa}{\mbox{O}(g_0^4 a)}
\newcommand{\icsw}{c_{\rm sw}}
\newcommand{\ict}{c_{\rm t}}
\newcommand{\icttil}{\tilde c_{\rm t}}
\newcommand{\icP}{c_{\rm\scriptscriptstyle P}}
\newcommand{\icA}{c_{\rm\scriptscriptstyle A}}
\newcommand{\icT}{c_{\rm\scriptscriptstyle T}}
\newcommand{\icV}{c_{\rm\scriptscriptstyle V}}
\newcommand{\ibP}{b_{\rm\scriptscriptstyle P}}
\newcommand{\ibA}{b_{\rm\scriptscriptstyle A}}
\newcommand{\ibT}{b_{\rm\scriptscriptstyle T}}
\newcommand{\ibV}{b_{\rm\scriptscriptstyle V}}
\newcommand{\ibm}{b_{\rm m}}
\newcommand{\ibmtil}{\tilde{b}_{\rm m}}
\newcommand{\ibmu}{b_\mu}

% Ginsparg-Wilson
\newcommand{\abar}{\kern1pt\overline{\kern-1pt a\kern-0.5pt}\kern1pt}
\newcommand{\abarhalf}{{\scriptstyle \frac{\abar}{2}}}
\newcommand{\psil}{\psi_{\mbox{\tiny L}}}

% Boldface and calligraphic capitals
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\bB}{{\mathbf{B}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\bN}{{\mathbf{N}}}
\newcommand{\bO}{{\mathbf{O}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\bQ}{{\mathbf{Q}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\bZ}{{\mathbf{Z}}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}

% Boldface three-vectors and funny caps for momenta
\newcommand{\vr}{\mathbf{r}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\ring}[1]{\mathaccent"7017 #1}

% Colours
\newcommand{\myred}[1]{\textcolor[rgb]{0.75,0,0}{#1}}
\newcommand{\mygrey}[1]{\textcolor[rgb]{0.5,0.5,0.5}{#1}}

